Achieving Hierarchy-Free Approximation for Bilevel Programs With Equilibrium Constraints

In this paper, we develop an approximation scheme for solving bilevel programs with equilibrium constraints, which are generally difficult to solve. Among other things, calculating the first-order derivative in such a problem requires differentiation across the hierarchy, which is computationally intensive, if not prohibitive. To bypass the hierarchy, we propose to bound such bilevel programs, equivalent to multiple-followers Stackelberg games, with two new hierarchy-free problems: a $T$-step Cournot game and a $T$-step monopoly model. Since they are standard equilibrium or optimization problems, both can be efficiently solved via first-order methods. Importantly, we show that the bounds provided by these problems -- the upper bound by the $T$-step Cournot game and the lower bound by the $T$-step monopoly model -- can be made arbitrarily tight by increasing the step parameter $T$ for a wide range of problems. We prove that a small $T$ usually suffices under appropriate conditions to reach an approximation acceptable for most practical purposes. Eventually, the analytical insights are highlighted through numerical examples.

==> test.tex <==
\begin{lemma}
\label{lm:iteration}
    For any $r, \eta > 0$, $\vs^t \in \bar \sR^{|\sK|}$, $\vp^t = q_r(\vs^t)$, and $\vp^t' \in \sP$, we have $\vp^t' = q_r(\vs^t + \eta \cdot c(\vp^t))$ if and only if 
    \begin{equation}
    \begin{split}
        \langle \nabla \phi_w(\vp^t_w) -  \nabla \phi_w(\vp^t_w'),  \vp_w - \vp^t_w' \rangle \leq r \cdot  \langle \eta \cdot c_w(\vp^t),  \vp_w - \vp^t_w'\rangle,  \quad \forall \vp_w \in \sQ_w(\vp^t_w), \quad \forall w \in \sW.
        \label{eq:p-2}
    \end{split}
    \end{equation}
\end{lemma}
\begin{proof}
    Denoting $\vs^t' = \vs^t + \eta \cdot c(\vp^t)$, Lemma \ref{lm:projection-logit} first implies that $\vp^t' = q_r(\vs^t')$ if and only if for all $w \in \sW$,
    \begin{equation}
    \begin{split}
        \vp^t_w' &= \argmin_{\vp_w \in \sP_w} \, D_w(\vp_w, \nabla \phi_w^*(-r \cdot \vs^t_w')) = \argmin_{\vp_w \in \sQ_w(\vp^t_w)} \, D_w(\vp_w, \nabla \phi_w^*(-r \cdot \vs^t_w')),
        \label{eq:fi-1}
    \end{split}
    \end{equation} 
    where the second equality holds because $D_w(\vp_w, \nabla \phi_w^*(-r \cdot  \vs^t_w')) < \infty$ if and only if $\vp_w \in \sQ_w(\vp^t_w)$ (see Lemma \ref{lm:kl-finite}). Subsequently, according to Lemma \ref{eg:optimization}, $\vp^t_w'$ solves Problem \eqref{eq:fi-1} if and only if
    \begin{equation}
        \langle \log(\vp^t_w') + 1 - \log(\nabla \phi_w^*(-r \cdot  \vs^t_w')),  \vp_w - \vp^t_w'\rangle \geq 0, \quad \forall \vp_w \in \sQ_w(\vp^t_w). 
        \label{eq:i-1}
    \end{equation}
    We then proceed to analyze the term $\log(\vp^t_w') + 1 - \log(\nabla \phi_w^*(-r \cdot  \vs^t_w'))$. First, we have $\nabla \phi_w(\vp^t_w') = \log(\vp^t_w') + 1$ by Lemma \ref{eg:entropy-dual}. Second,
    we can obtain that 
    \begin{equation}
    \begin{split}
        &\log(\nabla \phi_w^*(-r \cdot \vs^t_w'))  = \nabla \phi_w (\nabla \phi_w^*(-r \cdot \vs^t_w')) - 1 = -r \cdot \vs^t_w' - 1 \\
        &\qquad = -r \cdot \eta \cdot c_w(\vp^t) + \log(\vp^t_w) + \eva_w \cdot \vone_w - 1 =  -r \cdot \eta \cdot c_w(\vp^t) + \nabla \phi_w(\vp^t_w) + \eva_w \cdot \vone_w. 
        \label{eq:p-1}
    \end{split}
    \end{equation}
    where the first and second equalities come from Lemmas \ref{eg:entropy-dual} and \ref{lm:fenchel}, respectively, there must exists $\eva_w \in \sR^{|\sW|}$ such that the third equality holds  because of Lemma \ref{lm:difference-logit}, while the last equality is also derived from Lemma \ref{eg:entropy-dual}. Plugging both into Equation \eqref{eq:i-1}, we eventually obtain
    \begin{equation}
    \begin{split}
        \langle \nabla \phi_w(\vp^t_w) -  \nabla \phi_w(\vp^t_w'),  \vp_w - \vp^t_w' \rangle &\leq \langle r \cdot \eta \cdot c_w(\vp^t) - \eva_w \cdot \vone_w,  \vp_w - \vp^t_w'\rangle \\
        &= r \cdot  \langle \eta \cdot c_w(\vp^t),  \vp_w - \vp^t_w'\rangle,  \quad \forall \vp_w \in \sQ_w(\vp^t_w).
    \end{split}
    \end{equation}
    where the equality holds because $\langle \eva_w \cdot \vone_w,  \vp_w - \vp^t_w'\rangle = \eva_w \cdot (\langle \vone_w, \vp_w \rangle - \langle \vone_w, \vp^t_w' \rangle) = \eva_w \cdot (1 - 1) = 0$.
\end{proof}

